From Traditional to Deep Learning Approaches in Whole Slide Image Registration: A Methodological Review

Whole slide image (WSI) registration is an essential task for analysing the tumour microenvironment (TME) in histopathology. It involves the alignment of spatial information between WSIs of the same section or serial sections of a tissue sample. The tissue sections are usually stained with single or multiple biomarkers before imaging, and the goal is to identify neighbouring nuclei along the Z-axis for creating a 3D image or identifying subclasses of cells in the TME. This task is considerably more challenging compared to radiology image registration, such as magnetic resonance imaging or computed tomography, due to various factors. These include gigapixel size of images, variations in appearance between differently stained tissues, changes in structure and morphology between non-consecutive sections, and the presence of artefacts, tears, and deformations. Currently, there is a noticeable gap in the literature regarding a review of the current approaches and their limitations, as well as the challenges and opportunities they present. We aim to provide a comprehensive understanding of the available approaches and their application for various purposes. Furthermore, we investigate current deep learning methods used for WSI registration, emphasising their diverse methodologies. We examine the available datasets and explore tools and software employed in the field. Finally, we identify open challenges and potential future trends in this area of research.

==> temp.tex <==
% \newcolumntype{P}[1]{>{\RaggedRight\footnotesize}p{#1}}
% \begin{landscape}
% % \clearpage
% % \onecolumn
% \begin{longtable}{P{0.4in}P{0.9in} P{1.7in} P{1.5in} P{0.5in} P{1.3in} P{1.9in}} 
% \caption{Overview of papers using deep learning for WSI registration. \label{tab:alldeepworks}}\\
% \hline
% \centering  % centering table
% % \begin{tabular}{}
% % \hline
% Ref &Approach & Model  & dataset & Staining & Evaluation & Training Details \\ \hline

% Roy et al. \cite{roy2023deep} & (i) Translation-based and (ii) end-to-end registration  & (i) Modified Cycle GAN. (ii) CNN: 4-layer convolutional + BN +ReLU, followed by pooling and two layers of DeConv. & 76 breast cancer patients,  228 WSIs, with 3 serial WSIs from each patient.  & H\&E, Ki67, PHH3 & Qualitative and quantitative; NCC, SSIM,  NMI, Hausdorff distance and DSC& 60000 image patches randomly divided into training, validation and testing cohorts by patients at the ratio of 80:10:10. \\

% Xu et al. \cite{xu2020effective} & Translation-based registration & CycleGAN with constraint term  & Formalin-fixed paraffin-embedded tumour samples from 10 patients & H\&E, Ki67  & Qualitative: image/patch-level visualization and quantitative: comparison of the ratio of positive cells to all cells in a real Ki67 and the GAN Ki67 & 74492 (H\&E=34121, ki67= 33293) patches for training and 8427 patches (HE=4396 H\&E, KI67=4031) for test.  \\

% Daly et al. \cite{daly2021convolutional} & Feature extractor & Two modules: (i) a local classification CNN that extracts features from image patches and (ii) a global segmentation CNN operating on the extracted features.  & Three datasets with available gold-standard manual labels: (i) 235 Nissl-stained sequential coronal sections of the mouse brain from the Allen Brain Atlas \cite{wang2020allen}, and (ii) 416 WSI of HE cross-sections of mouse spinal cord \cite{maniatis2019spatiotemporal} and (iii) 12 whole-slide images of HE-stained cross-sections of human DLPFC collected across three neurotypical patients \cite{maynard2021transcriptome} & HE, Nissl & Accuracy, AUPRC and AUROC  & - \\

% Shao et al.\cite{shao2021prosregnet} &ii) Feature extraction and end-
% to-end registration & ResNEt-101 for feature extraction and a CNN regression model for end-to-end registration & MR and HE of 99 patients. & HE/MRI & Dice coefficient, the Hausdorff distance, and the mean landmark error & Training on internal cohort and evaluation using 53 patients from three different cohorts (an additional 12 from Cohort 1 and 41 from two public cohorts. \\

% % Wodzinski et al. \cite{wodzinski_aghsso_nodate}  &Approach & Model & ACROBAT 2022 dataset & H\&E, ER, PR, HER2, KI67 & Evaluation & comment \\

% Awan et al. \cite{awan2018deep} &  Feature extractor  & CNN (VGG\cite{simonyan2014very}) & ANHIR \cite{borovec2020anhir} and the non-public COMET (42 slides) datasets. Both have manual annotation and landmarks & H\&E, MLH1, MSH2, MSH6, PMS2, CK8/18  & Evaluation & comment \\ 
% Awan et al. \cite{awan2023deep}  &Feature extractor  & Model & dataset & Staining & Evaluation & comment \\
% Kondo et al. \cite{kondo_two_2022} &Approach & Model & dataset & Staining & Evaluation & comment \\
% Santi et al. \cite{santi_nemesis_2022} &Approach & Model & dataset & Staining & Evaluation & comment \\
% Jaderberg et al. \cite{jaderberg2015spatial} &Approach & Model & dataset & Staining & Evaluation & comment \\
% Zhao et al. \cite{zhao2019unsupervised} &Approach & Model & dataset & Staining & Evaluation & comment \\

% Gatenbee et al. \cite{gatenbee_virtual_2023} &Approach & Model & dataset & Staining & Evaluation & comment \\

% Budelmann et al. \cite{budelmann_histokatfusion_2022} &Approach & Model & dataset & Staining & Evaluation & comment \\
%  Marzahl et al. \cite{marzahl_robust_nodate} &Approach & Model & dataset & Staining & Evaluation & comment \\
%  \hline
%  \multicolumn{7}{P{8.2in}}{\small{\textbf{Abbreviations:} normalised cross correlation (NCC), structural similarity index measure (SSIM), and normalised mutual information (NMI), Dice similarity coefficient(DSC)}} \\ 
% % \end{tabular}
% % }
% \end{longtable}
% % \clearpage
% \twocolumn
% \end{landscape}
